Management Decisions in Manufacturing using Causal Machine Learning -- To Rework, or not to Rework?

In this paper, we present a data-driven model for estimating optimal rework policies in manufacturing systems. We consider a single production stage within a multistage, lot-based system that allows for optional rework steps. While the rework decision depends on an intermediate state of the lot and system, the final product inspection, and thus the assessment of the actual yield, is delayed until production is complete. Repair steps are applied uniformly to the lot, potentially improving some of the individual items while degrading others. The challenge is thus to balance potential yield improvement with the rework costs incurred. Given the inherently causal nature of this decision problem, we propose a causal model to estimate yield improvement. We apply methods from causal machine learning, in particular double/debiased machine learning (DML) techniques, to estimate conditional treatment effects from data and derive policies for rework decisions. We validate our decision model using real-world data from opto-electronic semiconductor manufacturing, achieving a yield improvement of 2 - 3% during the color-conversion process of white light-emitting diodes (LEDs).

==> fig/rework_flow.tex <==
\begin{tikzpicture}
  \begin{scope}[
    thick,
    every node/.style={minimum width=2.6cm, minimum height=0.8cm},
    % node types
    decision/.style={diamond,draw,top color=white,bottom color=yellow!20,,general shadow={fill=gray!60,shadow xshift=1pt,shadow yshift=-1pt}},
    block/.style={rectangle,draw,top color=white,bottom color=blue!10,general shadow={fill=gray!60,shadow xshift=1pt,shadow yshift=-1pt}},
    hidden/.style={rectangle,fill=white,text opacity=1,fill opacity=0},
  ]
    \node[block] (CONV) { apply converter };
    \node[block,below=0.5cm of CONV] (ICC) { measure (\(C_1\)) };
    \node[decision,aspect=2,below=0.5cm of ICC] (DECISION) {colour reached?};
    \node[block,right=of DECISION] (REW) { rework };
    \node[hidden,below=0.5cm of DECISION] (OTHER) { \(\ldots\) };
    \node[block,below=0.5cm of OTHER] (FT) { final test (\(C_2\)) };

    \path [->] (CONV) edge (ICC);
    \path [->] (ICC) edge (DECISION);
    \path [->] (DECISION) edge node[midway,above] {no} (REW);
    \path [->] (DECISION) edge node[midway,left] {yes} (OTHER);
    \path [draw, ->] (REW) |- (OTHER);
    \path [->] (OTHER) edge (FT);
  \end{scope}
\end{tikzpicture}


==> sections/abstract.tex <==
% Mainpoints:
% - causal model for rework decisions in manufacturing 
% - derive optimal rework policy depending on product and manchine properties
% - application on a challenging and unique problem in opto-electronic semiconductor manufacturing
\ABSTRACT{%
In this paper, we present a data-driven model for estimating optimal rework policies in manufacturing systems.
%setup
We consider a single production stage within a multistage, lot-based system that allows for optional rework steps.
While the rework decision depends on an intermediate state of the lot and system,
the final product inspection, and thus the assessment of the actual yield, is delayed until production is complete.
Repair steps are applied uniformly to the lot, potentially improving some of the individual items while degrading others.
The challenge is thus to balance potential yield improvement with the rework costs incurred.
%causal
Given the inherently causal nature of this decision problem,
we propose a causal model to estimate yield improvement.
We apply methods from causal machine learning,
in particular \abbreviation{DML}{double/debiased machine learning} techniques,
to estimate conditional treatment effects from data and derive policies for rework decisions.
%application
We validate our decision model using real-world data from opto-electronic semiconductor manufacturing,
achieving a yield improvement of $2-3\%$ during the color-conversion process of white \abbreviation{LEDs}{light-emitting diodes}.
%Rework plays an import role towards reaching the goal of zero-waste value chain, when applied to defective items.
}%


==> sections/discussion.tex <==
\section{Discussion}
\todo[inline]{I would include this in discussion and made a suggestion below. If it is okay for everybody, I would remove this whole Section.}
As production stages after the rework decision can have an influence on the 
final yield but do not affect the rework decision,
the causal setup described in section \ref{model:sec:causal_setting} 
should also include non-confounding system state stemming from them.
While such features can help to explain yield variation and thus to improve the estimation quality,
they have to be present at the time of decision-making.
Examples include manufacturing parameters defined in the product recipe,
or features that describe the condition of specific machines.
Since manufacturers tend to avoid variation in production the 
former are held mostly fixed after ramping of the product.
Thus, the effect of recipe variation on the yield -- while certainly present --
can hardly be estimated from production data alone.
Further, features that describe the machine condition,
have a limited validity due to equipment wear introduced or maintenance done
after the rework decision and before the actual machine usage.
In this regard a careful feature design is in order.

While the correction step is vastly simplified to a binary decision,
the framework could be adapted to allow for a set of specific or even parameterized repair decisions.
In the presented application this would mean to adjust certain spray gun settings
directly instead of deciding for a fixed setting when doing the rework step.
Further, an approach more in line with ZDM would be to adjust these settings 
before depositing the last regular layer. 
This has the drawback of always having at least two inspection steps at the phosphor deposition stage
-- one before and one after deposition of the final layer.


==> sections/methodology.tex <==
\section{Methodology}
As motivated in the previous section, in this scenario the treatment effect is heterogeneous with respect to covariates $X$. We will employ different approaches from conditional treatment effect estimation and optimal policy learning to learn a rework policy in this setting.

\subsection{Conditional Average Treatment Effects} \label{Sec:CATE}
Given a set of the covariates $\tilde{X}$ (not necessarily included in $X$), the CATE is defined as
$$\theta_0(\tilde{x}):=\mathbb{E}[g_0(1,X) - g_0(0,X)|\tilde{X}=\tilde{x}].$$
\citet{semenova2021debiased} propose to approximate $\theta_0(\tilde{x})\approx b(\tilde{x})^T\beta$ via a linear form, where $b(\tilde{x})$ is a $d$-dimensional basis vector of $\tilde{x}$. 
The idea is based on projecting the part $\psi_b(W_i,\eta)$ of the Neyman-orthogonal scores onto the predefined basis vector $b(\tilde{x})$.
The authors provide extensive theory to construct pointwise and jointly valid confidence intervals via Gaussian approximations.
As explained in Section \ref{Sec:Data}, being close to the color target might be well approximated via the first principal component of the production lot properties $X$. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/pca_obs.png}
    \caption{Principal components of the chip properties before treatment, treatment decision and observed outcome in the data for product type ``P1''. }
    \label{fig:pca_obs}
\end{figure}

To access the heterogeneity associated with the first principal component, we set $\tilde{X}$ to be the first principal component of the covariates $X$. Further, to allow for a flexible conditional treatment effect, we use a b-spline basis for $b(\tilde{x})$. The effect estimates combined with confidence intervals are displayed in Figure \ref{fig:cate_1d}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/CATE_1d_001.png}
    \caption{Estimation of the CATE along the first color point measurement. The horizontal dashed lines represent different policy thresholds $\gamma$.}
    \label{fig:cate_1d}
\end{figure}

As a positive CATE indicates improvements in yield, our estimated policy will be based on whether the effect on the yield surpasses some given threshold

$$\hat{\theta}(\tilde{x}) \ge \gamma,$$

where $\tilde{x}$ is the first principal component of $X$ and the threshold $\gamma>0$ can be used to incorporate costs and select rework groups at different effect levels.

Additionally considering the second principal component can contain further information about treatment effect heterogeneity and might improve the resulting policy. To be able to approximate the conditional effect flexibly based on the first two principal components, we rely on a tensor product of b-splines to construct our basis vector $b(\tilde{x})$. The resulting effect estimates are displayed in Figure \ref{fig:cate_2d}, where we omitted the confidence regions for clarity.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/CATE_2d_001.png}
    \caption{CATE with respect to both color point measurements.}
    \label{fig:cate_2d}
\end{figure}

It is visible that the first principal component captures the main heterogeneity of the treatment effect. Nevertheless, we will compare the difference in the policies in Section \ref{Sec:results}.

In both cases above, instead of using the effect estimate, using the lower bound of the confidence interval, will result in more conservative policy but account for the estimation uncertainty (see Appendix \ref{sec:confint}).
Additionally, one might consider the percentage of the reworked panels, to decide which threshold might be preferable to incorporate capacity constraints.

\subsection{Policy Leaning}
An alternative approach is to directly estimate a policy based on the part $\psi_b(W_i,\eta)$ in Equation \ref{eq:psi} as introduced by \citet{athey2021}. They propose to estimate the treatment assignment rule as
\begin{equation}
	\hat{\pi}=\argmax_{\pi\in\Pi}\frac{1}{n}\sum_{i=1}^{n}(2\pi(X_i)-1)\psi_b(W_i,\hat{\eta}).
	\label{eq:policy}
\end{equation}
Given a specified policy class $\Pi$ and the corresponding regret
\begin{align*}
R(\pi):=\max_{\pi'\in\Pi}\left\{\mathbb{E}[Y_i(\pi'(X_i))]\right\} - \mathbb{E}[Y_i(\pi(X_i))],
\end{align*}
the authors are able to derive regret bounds of order $1/\sqrt{n}$. 

The learning problem in Equation \ref{eq:policy} can be reformulated as a weighted classification problem
\begin{equation}
	\hat{\pi}=\argmax_{\pi\in\Pi}\frac{1}{n}\sum_{i=1}^{n}\lambda_i H_i(2\pi(X_i)-1),
\end{equation}
with weights $\lambda_i=|\psi_b(W_i,\hat{\eta})|$ and target $H_i = \textrm{sign}(\psi_b(W_i,\hat{\eta}))$. Thus, we define the space of possible policies $\Pi$ to be the class of depth-$m$ decision trees (see Figure \ref{fig:tree} as an example) with $m \in \{1,2\}$. Appendix \ref{app:rob} includes results for $\Pi$ being the class of linear decision boundaries after application of the radial basis function (rbf) kernel (using support vector machines).
To evaluate policies at different thresholds, we reduce the score by the desired threshold $\psi_b(W_i,\hat{\eta})-\gamma$ before classification.

\begin{figure}[h!]
    \centering
    \scalebox{0.75}{\input{fig/example_tree.tex}}
    \caption{Exemplary policy tree of depth $2$.}
    \label{fig:tree}
\end{figure}


==> sections/setting.tex <==
\section{Setting}
\subsection{Effect Identification}
As argued in Section \ref{Sec:Data} the rework decision is done based on the characteristics $X$. Consequently, conditioning on $X$ will close all backdoor paths between rework decision and yield. Put differently, we base our identification on conditional exogeneity, such that
$$Y(a)\perp A |X,$$
where $Y(a)$ denotes the potential outcome for $a\in \{0,1\}$ (see \cite{rubin2005}).
Under the assumptions above, the underlying causal structure can be represented by an interactive regression model (IRM):
\begin{align*}
    Y &= g_0(A,X) + U,\quad \mathbb{E}[U\mid X,A] =0,\\
    A &= m_0(X) + V,\quad \mathbb{E}[V\mid X] = 0,
\end{align*}
where the conditional expectations 
\begin{align}
    g_0(A,X) &= \mathbb{E}[Y\mid X, A],\label{eq:g_0}\\
    m_0(X) &= \mathbb{E}[A\mid X] = P(A=1\mid X)\label{eq:m_0}
\end{align}
are unknown and might be complex functions of $X$. In this structural equation model, the average treatment effect (ATE)
\begin{equation*}\label{ATE}
    \theta_{ATE} = \mathbb{E}[g_0(1,X)-g_0(0,X)]
\end{equation*}
as well as the \abbreviation{ATT}{average treatment effect of the treated}
\begin{equation*}\label{ATT}
    \theta_{ATT} = \mathbb{E}[g_0(1,X)-g_0(0,X)\mid A=1]
\end{equation*}
are identified. The work of \citet{chernozhukov2018} enables the use of machine learning (ML) algorithms such as random forest or boosting to obtain precise estimates of treatment effects combined with confidence intervals to access estimation uncertainty.

In double machine learning, inference is based on a method of moments estimator
\begin{equation}
    E[\psi(W;\theta_0,\eta_0)] = 0,
\end{equation}
with $\psi(W;\theta_0,\eta_0)$ being a Neyman-orthogonal score that identifies the causal parameter $\theta_0$ given ML estimates of the parameters or functions $\eta_0$ (referred to as nuisance). The Neyman-orthogonality property ensures robustness of the estimator against small perturbations in the ML nuisance estimates. Further, the usage of $k$-fold crossfitting safeguards against overfitting and enables to control the complexity of the estimator, leading to appealing properties such as $\sqrt{n}$-consistency and approximate normality.

In case of an IRM, the score for an ATE estimator is given by the linear form
\begin{align}
	\psi(W_i;\theta,\eta) :=&\ \psi_a(W_i,\eta)\theta + \psi_b(W_i,\eta)\\
	=&\ - \theta + g(1,X_i) - g(0,X_i) \nonumber \\
	 &\ + \frac{A_i(Y_i - g(1,X_i))}{m(X_i)} - \frac{(1-A_i)(Y_i - g(0,X_i))}{1-m(X_i)},
\label{eq:psi}
\end{align}
which is also known as augmented inverse propensity weighting (AIPW) \cite{robins1995}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{fig/ATE.png}
    \caption{Average treatment effect of reworking a chip lot and average treatment effect on the treated estimated by double machine learning.}
    \label{fig:ATE}
\end{figure}

Applied to the data, the estimates (see Figure \ref{fig:ATE}) suggest that for both products, the treatment effect is much higher on the treated than on the whole population. This emphasizes that treating all individual lots is not desirable in this setting, as the effect varies over the covariates $X$. \\

Figure \ref{fig:behavpol} shows the distribution of the main color point measure in $X$ for the treated and non-treated subsamples. There is no clear cut-off due to the reasons mentioned above. Ideally, there would be a policy in place that assigns the treatment to each production lot if the corresponding effect is above a set threshold (incorporating costs etc.). Our goal is to estimate a policy $\pi\in\Pi$, that maps individuals features $X_i \in \mathcal{X}$ to a treatment decision: $\pi : \mathcal{X} \rightarrow \{0, 1\}$, which incorporates the heterogeneity of the effect of the rework.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/histplot_per_bin.png}
    \caption{Distribution of the main color point measurement. Observations with a low value are already close to the target, thus they have a low treatment probability. Observations with a high value are therefore treated with a higher probability.}
    \label{fig:behavpol}
\end{figure}

During the rest of the paper, due to page constraints, we focus on the product type P1 (results for P2 can be found in Appendix \ref{app:L4}).

